The Hierarchical Subspace Iteration Method for Laplace--Beltrami Eigenproblems

Sparse eigenproblems are important for various applications in computer graphics. The spectrum and eigenfunctions of the Laplace--Beltrami operator, for example, are fundamental for methods in shape analysis and mesh processing. The Subspace Iteration Method is a robust solver for these problems. In practice, however, Lanczos schemes are often faster. In this paper, we introduce the Hierarchical Subspace Iteration Method (HSIM), a novel solver for sparse eigenproblems that operates on a hierarchy of nested vector spaces. The hierarchy is constructed such that on the coarsest space all eigenpairs can be computed with a dense eigensolver. HSIM uses these eigenpairs as initialization and iterates from coarse to fine over the hierarchy. On each level, subspace iterations, initialized with the solution from the previous level, are used to approximate the eigenpairs. This approach substantially reduces the number of iterations needed on the finest grid compared to the non-hierarchical Subspace Iteration Method. Our experiments show that HSIM can solve Laplace--Beltrami eigenproblems on meshes faster than state-of-the-art methods based on Lanczos iterations, preconditioned conjugate gradients and subspace iterations.

==> tables/SIM.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
%\begin{table}[]
%\resizebox{\linewidth}{!} 
%{
%	\begin{tabular}{|l|r|r||r|r|r|r|r|r|}
%	\hline
%	\multicolumn{1}{|c|}{}                        & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c||}{}                         & \multicolumn{2}{c|}{Random}                                 & \multicolumn{2}{c|}{2-Level}                          & \multicolumn{2}{c|}{Ours}                                    \\ \cline{4-9} 
%	\multicolumn{1}{|c|}{\multirow{-2}{*}{Model}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\#Vert}} & \multicolumn{1}{c||}{\multirow{-2}{*}{\#Eigs}} & \multicolumn{1}{c|}{iters} & \multicolumn{1}{p{0.35cm}|}{time}      & \multicolumn{1}{c|}{iters} & \multicolumn{1}{p{0.35cm}|}{time}     & \multicolumn{1}{c|}{iters}   & \multicolumn{1}{p{0.35cm}|}{time}     \\ \hline \hline
%%												&                                               & 50                                            &                            &                                &                            &                               &                              &                               \\ \cline{3-9} 
%%												&                                               & 100                                           &                            &                                &                            &                               &                              &                               \\ \cline{3-9} 
%%	\multirow{-3}{*}{Ball}                        & \multirow{-3}{*}{90k}                         & 250                                           &                            &                                &                            &                               &                              &                               \\ \hline
%												&                                               & 50                                            & {\color[HTML]{000000} 15}  & {\color[HTML]{000000} 193.2}   & {\color[HTML]{000000} 11}  & {\color[HTML]{000000} 143.0}  & {\color[HTML]{000000} 5,4,4} & {\color[HTML]{000000} 89.3}   \\ \cline{3-9} 
%												&                                               & 100                                           & {\color[HTML]{000000} 14}  & {\color[HTML]{000000} 392.3}   & {\color[HTML]{000000} 12}  & {\color[HTML]{000000} 342.4}  & {\color[HTML]{000000} 4,5}   & {\color[HTML]{000000} 190.2}  \\ \cline{3-9} 
%	\multirow{-3}{*}{Fertility}                   & \multirow{-3}{*}{241k}                        & 250                                           & {\color[HTML]{000000} 15}  & {\color[HTML]{000000} 1120.8}  & {\color[HTML]{000000} 11}  & {\color[HTML]{000000} 841.3}  & {\color[HTML]{000000} 5,5}   & {\color[HTML]{000000} 498.3}  \\ \hline
%												&                                               & 50                                            & {\color[HTML]{000000} 14}  & {\color[HTML]{000000} 436.7}   & {\color[HTML]{000000} 11}  & {\color[HTML]{000000} 351.1}  & {\color[HTML]{000000} 5,3,4} & {\color[HTML]{000000} 226.7}  \\ \cline{3-9} 
%												&                                               & 100                                           & {\color[HTML]{000000} 14}  & {\color[HTML]{000000} 977.5}   & {\color[HTML]{000000} 11}  & {\color[HTML]{000000} 787.5}  & {\color[HTML]{000000} 6,4,4} & {\color[HTML]{000000} 424.9}  \\ \cline{3-9} 
%	\multirow{-3}{*}{Oil pump}                    & \multirow{-3}{*}{570k}                        & 250                                           & {\color[HTML]{000000} 14}  & {\color[HTML]{000000} 2630.2}  & {\color[HTML]{000000} 11}  & {\color[HTML]{000000} 2120.4} & {\color[HTML]{000000} 4,5}   & {\color[HTML]{000000} 1337.5} \\ \hline
%												&                                               & 50                                            & {\color[HTML]{000000} 14}  & {\color[HTML]{000000} 655.7}   & {\color[HTML]{000000} 11}  & {\color[HTML]{000000} 475.5}  & {\color[HTML]{000000} 4,4,4} & {\color[HTML]{000000} 372.3}  \\ \cline{3-9} 
%												&                                               & 100                                           & {\color[HTML]{000000} 14}  & {\color[HTML]{000000} 1453.3}  & {\color[HTML]{000000} 10}  & {\color[HTML]{000000} 983.9}  & {\color[HTML]{000000} 4,4,4} & {\color[HTML]{000000} 655.2}  \\ \cline{3-9} 
%	\multirow{-3}{*}{Ramses}                      & \multirow{-3}{*}{830k}                        & 250                                           & \multicolumn{2}{r|}{{\color[HTML]{000000} not converging}} & {\color[HTML]{000000} 11}  & {\color[HTML]{000000} 2834.7} & {\color[HTML]{000000} 6,4,4} & {\color[HTML]{000000} 1572.7} \\ \hline
%\end{tabular}
%}
%\caption{Comparison of our multilevel eigensolver to classical SIM with random initial vectors and 2-level SIM, 
%which is a classic SIM with good quality initial vectors from our reduced eigenfunctions.}
%	\label{tab:variousSIM}
%\end{table}

\begin{table}[t]
\resizebox{\linewidth}{!} 
{
	\begin{tabular}{|l|r||r|r|r|r|}
	\hline
	\multicolumn{1}{|c|}{}                        & \multicolumn{1}{c||}{}                         & \multicolumn{2}{c|}{Orig. SIM}                                 & \multicolumn{2}{c|}{Ours}                                    \\ \cline{3-6} 
	\multicolumn{1}{|c|}{\multirow{-2}{*}{Model (\#Vert)}} & \multicolumn{1}{c||}{\multirow{-2}{*}{\#Eigs}} & \multicolumn{1}{c|}{iters} & \multicolumn{1}{p{0.35cm}|}{time}      & \multicolumn{1}{c|}{iters}   & \multicolumn{1}{p{0.35cm}|}{time}     \\ \hline \hline
															%	& 50                                            & {11}  						& {24.6(49.7)}    				& {D|2} 				& {10.0} \\ \cline{2-6} 
																& 100                                           & {11}  						& {62.2(111.2)}   				& {D|2} 				& {15.2} \\ \cline{2-6} 
																& 250                                           & {11}  						&{173.1(300.0)}   				& {D|3} 				& {52.6} \\ \cline{2-6} 
	\multirow{-3}{*}{\parbox{1.5cm}{Ch.Dragon (127k)}}          & 1000                                          & {--}  						&{-(-)}   						& {---} 				& {----} \\ \hline
															%	& 50                                            & {11}  						& { 48.1(94.0)}   				& {D|2} 				& {18.7} \\ \cline{2-6} 
																& 100                                           & {11}  						& {117.7(243.4)}  				& {D|2} 				& {29.3} \\ \cline{2-6} 
																& 250                                           & {11}  						& {388.2(597.7)}  				& {D|3} 				&{100.9} \\ \cline{2-6} 
	\multirow{-3}{*}{\parbox{1.5cm}{Fertility (241k)}}          & 1000                                          & {25}  						&{3112.1(5129.4)}  				& {D|5} 				&{531.0} \\ \hline
																& 50                                            & {--}  						& {-----------}   				& {D|2|1} 				& {71.7} \\ \cline{2-6} 
																& 100                                           & {--}  						& {-----------}   				& {D|2|1} 				& {91.0} \\ \cline{2-6} 
	\multirow{-3}{*}{\parbox{1.5cm}{Oil pump (570k)}}           & 250                                           & {--}  						& {------------}  				& {D|3|2} 				&{235.2} \\ \hline
\end{tabular}
}
\caption{Comparison of our hierarchical eigensolver to the classical SIM with random initial vectors, on models with varying number of vertices. (Tolerance is $1\times10^{-3}$).}
	\label{tab:variousSIM}
\end{table}


==> tables/constantWeight.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\resizebox{0.75\linewidth}{!} 
{
	\begin{tabular}{|l|r|r|r|r|r|r|}
	\hline
	\multicolumn{1}{|c|}{\multirow{2}{*}{Model}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#Vert}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#Eigs}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Piecewise\\ constant\end{tabular}} & \multicolumn{2}{c|}{Ours}                              \\ \cline{4-7} 
	\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{iters}               & \multicolumn{1}{c|}{time}              & \multicolumn{1}{c|}{iters} & \multicolumn{1}{c|}{time} \\ \hline
	\multirow{3}{*}{Ball}                        & \multirow{3}{*}{90k}                         & 50                                           & 16,20                                    & 88.4                                   & 9,6                        & 38.7                      \\ \cline{3-7} 
												&                                              & 100                                          & 9,7                                      & 72.6                                   & 5,3                        & 42.2                      \\ \cline{3-7} 
												&                                              & 250                                          & 10,9                                     & 237.0                                  & 8,5                        & 173.1                     \\ \hline
	\multirow{3}{*}{Sphere}                      & \multirow{3}{*}{160k}                        & 50                                           & 12,9,8                                   & 94.4                                   & 8,5,4                      & 62.7                      \\ \cline{3-7} 
												&                                              & 100                                          & 8,8                                      & 180.9                                  & 4,5                        & 127.0                     \\ \cline{3-7} 
												&                                              & 250                                          & 10,9                                     & 527.7                                  & 5,5                        & 330.8                     \\ \hline
	\multirow{3}{*}{Fertility}                   & \multicolumn{1}{l|}{\multirow{3}{*}{241k}}   & 50                                           & 11,9,8                                   & 135.2                                  & 6,4,5                      & 100.7                     \\ \cline{3-7} 
												& \multicolumn{1}{l|}{}                        & 100                                          & 10,9                                     & 312.7                                  & 5,5                        & 196.0                     \\ \cline{3-7} 
												& \multicolumn{1}{l|}{}                        & 250                                          & 10,9                                     & 756.8                                  & 5,6                        & 563.9                     \\ \hline
	\end{tabular}
}
\caption{Comparison of our construction to the hierarchy constructed by \cite{xian2019scalable}, both without any shifting strategy.
	In most cases, our multilevel requires approximately half number of iterations compared to their hierarchy with piecewise constant weight.}
	\label{tab:weight}
\end{table}

==> tables/decay.tex <==
\begin{table}[]
\resizebox{\linewidth}{!} 
{
	\begin{tabular}{|l|r|r|c|r|c|r|c|r|c|r|c|r|c|}
	\hline
	\multicolumn{1}{|c|}{\multirow{2}{*}{Model}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#Eigs}} & \multicolumn{2}{c|}{4}             & \multicolumn{2}{c|}{5}             & \multicolumn{2}{c|}{7}             & \multicolumn{2}{c|}{10}            & \multicolumn{2}{c|}{15}            & \multicolumn{2}{c|}{20}            \\ \cline{3-14} 
	\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\#Lvl} & Time  & \multicolumn{1}{c|}{\#Lvl} & Time  & \multicolumn{1}{c|}{\#Lvl} & Time  & \multicolumn{1}{c|}{\#Lvl} & Time  & \multicolumn{1}{c|}{\#Lvl} & Time  & \multicolumn{1}{c|}{\#Lvl} & Time  \\ \hline
	\multirow{3}{*}{Balls}                       & 50                                           & 5                          & 61.7  & 5                          & 49.1  & 4                          & 43.6  & 3                          & 36.0  & 3                          & 32.0  & 3                          & 31.3  \\ \cline{2-14} 
												& 100                                          & 5                          & 68.3  & 4                          & 55.9  & 4                          & 50.2  & 3                          & 40.9  & 3                          & 38.6  & 2                          & 29.2  \\ \cline{2-14} 
												& 250                                          & 4                          & 218.5 & 4                          & 210.6 & 3                          & 173.1 & 3                          & 165.5 & 2                          & 195.7 & 2                          & 154.2 \\ \hline
	\multirow{3}{*}{Blade}                       & 50                                           & 6                          & 102.7 & 5                          & 81.8  & 4                          & 65.9  & 4                          & 58.3  & 3                          & 51.0  & 3                          & 58.4  \\ \cline{2-14} 
												& 100                                          & 5                          & 179.3 & 5                          & 164.9 & 4                          & 130.2 & 3                          & 110.7 & 3                          & 95.7  & 3                          & 93.4  \\ \cline{2-14} 
												& 250                                          & 5                          & 520.9 & 4                          & 438.2 & 3                          & 362.3 & 3                          & 346.7 & 3                          & 325.2 & 2                          & 598.1 \\ \hline
	\end{tabular}
}
\caption{The effect of varying decay rate to the performance of the multilevel eigensolver.}
	\label{tab:decay}
\end{table}

==> tables/lanczos.tex <==
\begin{table}[]
\resizebox{0.975\linewidth}{!} 
{
	\begin{tabular}{|c|r||r|r|r|r|}
	\hline
	\multicolumn{1}{|c|}{Model(\#Vert)} 				& \multicolumn{1}{c||}{\#Eigs} & \multicolumn{1}{c|}{\textsc{SpectrA}} & \multicolumn{1}{c|}{MH} & \multicolumn{1}{c|}{\textsc{Matlab}} & \multicolumn{1}{c|}{Ours} \\ \hline \hline
	\multirow{4}{*}{\parbox{1.5cm}{Dragon (160k)}}      & 50                         &                              &    12.3                 &   12.1                      &  12.0                      \\ \cline{2-6} 
														& 250                        &                              &    88.0                 &   63.8                      &  32.5                      \\ \cline{2-6} 
														& 1000                       &                              &                         &  890.3                      & 182.1                      \\ \cline{2-6} 
														& 2500                       &                              &                         & 5733.9                      & 362.7                      \\ \hline
	\multirow{3}{*}{\parbox{1.5cm}{Rocker-Arm (270k)}} 	& 50                         &                              &                         &   21.7                      &  36.1                      \\ \cline{2-6} 
														& 250                        &                              &                         &  131.7                      &  82.6                      \\ \cline{2-6} 
														& 1000                       &                              &                         & 1423.5                      & 405.6                      \\ \cline{2-6}
														& 2500                       &                              &                         &                             &1287.0                      \\ \hline 
	\multirow{3}{*}{\parbox{1.5cm}{Mechanics (660k)}}  	& 50                         &                              &                         &   70.6                      &  87.5                      \\ \cline{2-6} 
														& 250                        &                              &                         &  365.4                      & 231.5                     \\ \cline{2-6} 
														& 1000                       &                              &                         & 3995.5                      & 979.1                     \\ \hline
	\end{tabular}
}
\caption{Timing comparison (in seconds) of our HSIM eigensolver to other state-of-the-art implementation of Lanczos methods.
	The HSIM is significantly faster than SpectrA for similar accuracy, and faster than MH and Matlab while producing more accurate results.
	The maximum relative $L^2$-norm residual for all solvers is $1\times10^{-2}$, except Matlab with value of $0.99$.
	}
\label{tab:lanczos}
\end{table}

==> tables/shift-noshift.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|l|r|r||r|r|r|r|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Model}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#Vert}} & \multicolumn{1}{c||}{\multirow{2}{*}{\#Eigs}} & \multicolumn{2}{c|}{No shift}                          & \multicolumn{2}{c|}{With shift}                        \\ \cline{4-7} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c||}{}                        & \multicolumn{1}{c|}{iters} & \multicolumn{1}{c|}{time} & \multicolumn{1}{c|}{iters} & \multicolumn{1}{c|}{time} \\ \hline \hline
\multirow{3}{*}{Ch. Dragon}                  & \multirow{3}{*}{127k}                        & 50                                           & 9,5,4                      & 39.2                      & 7,4,4                      & 36.9                      \\ \cline{3-7} 
                                             &                                              & 100                                          & 5,5                        & 81.30                     & 5,4                        & 70.0                      \\ \cline{3-7} 
                                             &                                              & 250                                          & 7.5                        & 223.3                     & 5,4                        & 173.9                     \\ \hline
\multirow{3}{*}{Mechanics?}                  & \multirow{3}{*}{660k}                        & 50                                           & 5,5,6                      & 298.7                     & 4,4,5                      & 247.7                     \\ \cline{3-7} 
                                             &                                              & 100                                          & 6,5,6                      & 597.8                     & 5,4,5                      & 517.6                     \\ \cline{3-7} 
                                             &                                              & 250                                          & 8,5,6                      & 1617.6                    & 7,4,5                      & 1470.0                    \\ \hline
\end{tabular}
\caption{A good approximation of eigenvalues allows us to shift to appropriate index, 
	thus reducing the number of iterations to achieve certain target convergence rate, e.g. $1\times{10^{-4}}$ in this example.}
	\label{tab:shift}
\end{table}
